Dark matter as the origin of neutrino mass in the inverse seesaw mechanism

We propose that neutrino masses are "seeded" by a dark sector within the inverse seesaw mechanism. This way we have a new, "hidden", variant of the scotogenic scenario for radiative neutrino masses. We discuss both explicit and dynamical lepton number violation. In addition to invisible Higgs decays with majoron emission, we discuss in detail the pheneomenolgy of dark matter, as well as the novel features associated to charged lepton flavour violation, and neutrino physics.

==> Makefile <==
FILENAME=inv-scotogenic
LATEX = pdflatex
BIBTEX = bibtex
PDFTOPS = pdftops
AR = acroread
GV = gv
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

PSFILE = inv-scotogenic.ps 
PDFFILE = inv-scotogenic.pdf

COPY = if test -r inv-scotogenic.toc; then cp inv-scotogenic.toc inv-scotogenic.toc.bak; fi 
RM = /bin/rm -f

CLEAN=rm -f inv-scotogenic.aux inv-scotogenic.log inv-scotogenic.dvi inv-scotogenic.toc inv-scotogenic.out inv-scotogenic.blg inv-scotogenic.mtc inv-scotogenic.mtc1 inv-scotogenic.rel inv-scotogenic.vrb inv-scotogenic.end inv-scotogenic.spl *.aux *~ \#*

WARNING=egrep -i "(Reference|Citation).*undefined" inv-scotogenic.log ; true

HELP=cat /home/jv/bin/help/MakePDFLatexMakefile.help

main:	inv-scotogenic.tex pdf

pdf:	$(PDFFILE)
	$(WARNING)  

all:	$(PDFFILE) $(PSFILE)
	$(WARNING)  

ps:	$(PSFILE) 
	$(WARNING)

gv:	$(PSFILE)
	$(GV) $(PSFILE) &
	$(WARNING)

	$(WARNING)

ar:	$(PDFFILE)
	$(AR) $(PDFFILE) &

%.pdf:	%.tex
	python3.6 /usr/local/bin/PhysBiblio.exe tex bibliography.bib './inv-scotogenic.tex' 
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ;true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if [  'cmp -s $*.toc $*.toc.bak'  ]; then $(LATEX) $< ; fi
	$(RM) $*.toc.bak

%.ps:	%.pdf
	$(PDFTOPS) $<

clean:	
	$(CLEAN)

realclean: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).pdf $(FILENAME).bbl

help:
	$(HELP)

complete: realclean pdf clean


